Game Design for Eliciting Distinguishable Behavior

The ability to inferring latent psychological traits from human behavior is key to developing personalized human-interacting machine learning systems. Approaches to infer such traits range from surveys to manually-constructed experiments and games. However, these traditional games are limited because they are typically designed based on heuristics. In this paper, we formulate the task of designing \emph{behavior diagnostic games} that elicit distinguishable behavior as a mutual information maximization problem, which can be solved by optimizing a variational lower bound. Our framework is instantiated by using prospect theory to model varying player traits, and Markov Decision Processes to parameterize the games. We validate our approach empirically, showing that our designed games can successfully distinguish among players with different traits, outperforming manually-designed ones by a large margin.

==> defn.tex <==
\section{Informative MDP Design}
\begin{definition}
(Markov Decision Process) A Markov Decision Process $\mathcal{M}$ is specified by $(\mathcal{S}, \mathcal{A}, T, r, \gamma)$ where $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space. For each state-action pair $(s,a)$, $T(s,a)$ gives a probability distribution over the next state. $r: \mathcal{S} \to \mathbb{R}$ is a reward function. $\gamma \in (0,1)$ is a discount factor.
\end{definition}

For all $s \in \mathcal{S}$, a policy $\pi(\cdot|s)$ defines a distribution over actions at state $s$. A (optimal) policy for an MDP $\mathcal{M}$ is denoted as $\pi_\mathcal{M}$.  A Trajectory generated according to $\pi_\mathcal{M}$ is denoted as $\tau_{\pi_\mathcal{M}}$.

When perceiving the same MDP $\mathcal{M}$, humans tend to have distinctive ways of interpreting it. Such a distortion $f$ maps $\mathcal{M}$ to another MDP $\mathcal{M}'$ through changing the transition $T$ and the reward function $r$. 
Our goal is to design a base $\mathcal{M}$ such that the policy $\pi_{f(\mathcal{M})}$ is distinguishable for different $f$.

\begin{definition}
(Informative MDP Design) 
Given $\mathcal{S}, \mathcal{A}$ and $\gamma$, a distribution of transformations $Y$, our goal is to 
$$\arg \max_{T, r} I(Y; \pi_{Y(\mathcal{M})})$$
where $\mathcal{M} = (\mathcal{S}, \mathcal{A}, T, r, \gamma)$, $Y(\mathcal{M})$ is a distribution over the transformed MDPs, $\pi_{Y(\mathcal{M})}$ is a distribution over policies induced by the transformed MDPs.

\end{definition}
